Autonomous Apple Fruitlet Sizing with Next Best View Planning

In this paper, we present a next-best-view planning approach to autonomously size apple fruitlets. State-of-the-art viewpoint planners in agriculture are designed to size large and more sparsely populated fruit. They rely on lower resolution maps and sizing methods that do not generalize to smaller fruit sizes. To overcome these limitations, our method combines viewpoint sampling around semantically labeled regions of interest, along with an attention-guided information gain mechanism to more strategically select viewpoints that target the small fruits' volume. Additionally, we integrate a dual-map representation of the environment that is able to both speed up expensive ray casting operations and maintain the high occupancy resolution required to informatively plan around the fruit. When sizing, a robust estimation and graph clustering approach is introduced to associate fruit detections across images. Through simulated experiments, we demonstrate that our viewpoint planner improves sizing accuracy compared to state of the art and ablations. We also provide quantitative results on data collected by a real robotic system in the field.

==> dep_4_Preliminaries.tex <==

\subsection{ROI Point Cloud Extraction}
We extract a semantically labelled point cloud using segmented fruitlets and estimated disparities. Fruitlet segmentation is performed using a Mask-RCNN~\cite{maskrcnn2017} instance segmentation network with a ResNet-101~\cite{resnet} backbone. The network was trained on 400 manually labeled 1080$\times$1440 images for 25 epochs on an NVIDIA GeForce RTX 3070. Disparity estimation was performed using a pre-trained RAFT-Stereo \cite{lipson2021raft} faster implementation network, with an inference time of approximately 0.7s per image.

To reduce noise, the point cloud undergoes a two-stage filtering process. First, a bilateral filter is used to smooth the depths while preserving edges. Second, we apply a depth discontinuity filter presented in \cite{6906903} to help mitigate the effect of discontinuities on \todo{somehow add figure?} depth. 

%Here we will discuss Octomap, ROI Octomap, and Attention Region

%%%%%%%%
\subsection{3D Map Representation}
Discuss 3D map. When describing raycasting show visualization like you do below to make it relateable.

\subsection{Attention Region}
Discuss Attention

To focus attention on a certain region in space
Attention not learned
Similar to how attention in ML focusses weights on things, this is focus on area in space

Can say removed exploration sampling because this is not exploration nbv

"attention" typically refers to the mechanism or strategy that an autonomous system uses to focus on specific regions or objects within its environment.
In summary, attention in the context of active perception and viewpoint planning is a mechanism that enables autonomous systems to intelligently focus their sensory resources on regions or objects that are most relevant to their tasks and goals. It plays a crucial role in optimizing perception, decision-making, and action in complex and dynamic environments.

Future work apply attention and exploration based sampling

\begin{align}
    I(x)&= 
    \begin{cases}
        1,& \text{if } x= \text{unknown }\\
        0,              & \text{otherwise}
    \end{cases} \label{ig_0} \\[5pt]
     N_{A, r} &= \sum_{x\in X_r\cap A}1 \label{ig_1} \\[5pt]
     N_{A, u, r} &= \sum_{x\in X_r\cap A} I(x) \label{ig_2} \\[5pt]
    IG_r &= 
    \begin{cases}
        \frac{N_{A, u, r}}{N_{A, r}},& \text{if } N_{A, r} > 0\\[5pt]
        0,              & \text{otherwise}
    \end{cases} \label{ig_3} \\[5pt]
    IG &= \frac{1}{|R|}\sum_{r \in R} IG_r \label{ig_4}
\end{align}

==> dep_introduction.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}

\todo{actually though come up with your own citations, you can't copy zaenker like this}
With population growth, climate change, and labor shortages on the rise, the global food supply is continuously facing more and more pressure. As a result, agriculturalists are actively looking to adopt robotics solutions to improve efficiency and reduce the time and effort required to perform labor-intensive tasks. Among these tasks is autonomous crop inspection, which is integral for precision agriculture as it enables farmers to make smarter and more informed decisions for a variety of downstream processes including \todo{do I need to cite these? I don't think so. Wait I can} quality control, disease and pest management, pruning, and harvesting. Autonomous crop inspection systems have been deployed for several different tasks including \todo{make your own, could use T-RO ones or find some. And cite} mapping rows of crops \cite{rs12091357, STEFAS2019104814}, \todo{cite} individual plant monitoring, and \todo{cite} fruit sizing. 

In this work, we present a method to autonomously inspect apple fruitlets by measuring their sizes. An apple fruitlet is a very young apple that has formed on the apple tree shortly after pollination. Apple fruitlets tend to grow in clusters, where a cluster is a group of fruitlets that grow out of the same bud, with typically 3-6 fruitlets per cluster as shown in \todo{figure, like with fruitlet, cluster, numbering labelling, like thesis but different} Fig.~\ref{fig:cluster_example}. Measuring the sizes of apple fruitlets is important because apple growers compare the diameters of fruitlets in a cluster to determine when to apply chemical thinners to their trees in order to optimize their yearly yield \cite{greene2013development}. Manually sizing fruitlets is labor-intensive, as %hand
calipers have to be used to record the diameters of approximately 500 fruitlets per varietal at a minimum of twice per thinning application. As a result, apple growers are looking for autonomous solutions.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/bb_and_fruitlet.png}
    \put(-197, 127){\scriptsize Stereo Camera}
    \put(-174, 116){\scriptsize UR5}
    \put(-156, 111){\scriptsize Linear Slider}
    \caption{Left: Stereo camera attached to a 7 DoF robotic arm. Right: Example of a fruitlet cluster with AprilTag hung in near-proximity for identification.}
    \label{fig:bb_and_fruitlet}
\end{figure}

COMMENTING OUT FOR SPACE PURPOSES ONLY TODO ADD BACK IN WHEN YOU DO INTRO.
In order to autonomously measure the diameters of apple fruitlets, images have to be captured that will allow the fruits to be subsequently sized. This task is challenging because fruitlets grow in very occluded environments. There are leaves, branches, and wind, and often fruitlets in the same cluster will occlude one another (Fig.~\ref{fig:cluster_example}). The robot needs to be able to reason about the environment and determine the optimal viewpoints to capture images. We achieve this using a next-best-view (NBV) planning approach targeted towards sizing smaller fruit. State-of-the-art NBV planners in agriculture are designed to size larger fruit that are sparsely populated. They rely on low-resolution maps


Previous NBV planners in agriculture are designed to size larger fruit that are sparsely populated. They rely on low-resolution maps and naive association methods that do not generalize across smaller fruit sizes. To overcome these limitations, we present an NBV planning approach that utilizes regions of interest for viewpoint sampling and an attention-guided mechanism for calculating information gain. In addition, we integrate a dual-map representation of the environment that significantly speeds up expensive ray casting operations while maintaining finer occupancy information. To address the challenges of data association in the presence of wind and sensor error, we introduce a robust estimation and graph clustering approach. We demonstrate that our planning method improves sizing accuracy compared to another state-of-the-art planner used in agriculture. Our main contributions are 

\begin{itemize}
    \item A novel next-best-view planner that uses coarse and fine occupancy maps with an attention-guided information gain metric to capture images of smaller fruit.
    \item A robust estimation and graph clustering approach to associate fruitlet detections across images in the presence of wind and sensor error. 
    \item Quantitative evaluation on data collected by a real robotic system in a commercial apple orchard.
\end{itemize}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/nbv_system_overview.png}
    \put(-275, 118){(a)}
    \put(-362, -11){(b)}
    \put(-112, -11){(c)}
    \caption{Overview of our next-best-view planning and sizing pipeline.
    \label{fig:nbv_full_pipeline}}
\end{figure*}
\newpage

% images have to be captured and then the fruits subsequently

% Capturing \todo{don't like this word} useful images requires sp

% Then do what Zaenker did, can't do fixed camera, need active planning. state of the art nbv planners don't work

% In order to autonomously inpsect crops,

% advanced automated agricultural applications such as fruit
% picking or targeted crop spraying require spatial informa-
% tion about plants. With a fixed sensor setup, generating a
% 3D model can be difficult, as parts of the plants are typically
% occluded. Especially plants with a large number of leaves
% are challenging. Therefore, having a mobile sensor placed
% on a robotic arm to move it around and avoid occlusions is
% a promising solution. However, in order to know where to
% place the sensor, viewpoints have to be planned first.

% owever, frequent
% occlusion of fruits and the variation in their position on
% plant structures make their reliable perception a challenging
% task. 

% As fruitlets grow and fall off etc. positions are unkown, this is an active perception problem. Explain why use NBV active perception in agriculture, cite papers. 

% Say state of the art viewpoint planners are dedicated towards sizing larger fruit. Explain your schpeel

% Say what you do and your contributions. 

==> ep_2_Related_Work.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
There have previous works dedicated towards viewpoint planning in agriculture, where approaches either local sensor information or build a volumetric map of the environment to determine the next best camera pose. 

\todo{whole section needs redoing} Next-best-view (NBV) planners are used to determine the next best camera pose that maximizes information gain. Alternative to coverage path planners, which rely on prior information to compute optimal camera poses to cover the area of known static maps \todo{CITE} CITE %\cite{8239550, jing2019coverage, cpp_ag_field, 10050562, cpp_agg_wheeled, Driscoll2011CompleteCP}
, NBV planners are used to explore unknown and dynamic environments. They rely on information gain metrics \todo{CITE} CITE %\cite{7487527, delmerico} 
to evaluate candidate viewpoints to effectively explore unknown areas of interest. 

There have been previous works dedicated towards NBV planning in agriculture, where approaches either use only current sensor information or build a volumetric map of the environment to determine the next-best-view. Examples of the former include the work of \todo{CITE} CITE %\cite{lehnert20183d},
who use a 3D camera array to capture images to size a target fruit of interest. The next best camera pose is selected by computing a gradient to determine the optimal direction in which the visibility of the target is increased. While this method is effective at avoiding local occlusions, it cannot extend globally when multiple targets need to be imaged. As well, in \todo{CITE} CITE %\cite{8206500}
, a viewpoint planning approach is presented to count the number of apples in a cluster. They determine the optimal camera pose by maximizing entropy of a set of world hypotheses informed by previous images. However, the method makes simplified occlusion assumptions that do not extend well when sizing smaller fruit. 

More commonly, volumetric-based planning approaches have been adopted in agriculture, where occupancy information stored inside a volumetric map is used to guide the planning process. These methods often combine occupancy and region of interest (ROI) information when determining the next best camera pose. In the work of \todo{CITE} CITE %\cite{8793560}
, detected ROIs in the form of segmented apples are used to evaluate viewpoints based on a weighted sum of exploration information. This information is then used as input into a Decentralized Monte Carlo Tree Search \todo{CITE} CITE %\cite{decmcts}
planner to plan a sequence of viewpoints for multiple robot arms. However, computing a sequence of viewpoints can be computationally expensive. Zaenker \textit{et al.} \todo{CITE} CITE %\cite{nbv_zaenker}
address this issue by using ROIs to more informatively sample viewpoints. The information gain for each viewpoint is then approximated by casting rays through the volumetric map. While this is a more greedy approach, as only single points are evaluated instead of a complete path, the computational cost is much less. The authors of \todo{CITE} CITE %\cite{new_zaenker} 
try to further reduce the computational complexity by using automated shape completion along with a viewpoint dissimilarity metric to estimate information gain, replacing the need for ray casting. However, this does not extend well to smaller fruit, where shape completion methods traditionally fail as a result of the inability to capture enough of the fruit's surface. 

An attention-guided NBV planning approach is presented by Burusa \textit{et al.} \todo{CITE} CITE %\cite{burusa2022attentiondriven}
, where attention regions defined around different plant components are used to restrict which voxels contribute to the information gain. The authors demonstrate that thid led to improved results regarding both reconstruction accuracy and speed. However, the location and size of the attention regions were assumed to be prior knowledge, which is not the case when sizing unknown fruit. As well, they did not consider ROI information when viewpoint sampling, and sample viewpoints on a cylindrical sector which was also assumed to be known beforehand.

%TODO make sure to include your inhand camera too I suppose

==> ieee_examples.tex <==
\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
\item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

\subsection{Some Common Mistakes}
\begin{itemize}


\item The word ÒdataÓ is plural, not singular.
\item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
\item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
\item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
\item Do not confuse ÒimplyÓ and ÒinferÓ.
\item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
\item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.
